A Prototypical Expert-Driven Approach Towards Capability-Based Monitoring of Automated Driving Systems

Supervising the safe operation of automated vehicles is a key requirement in order to unleash their full potential in future transportation systems. In particular, previous publications have argued that SAE Level 4 vehicles should be aware of their capabilities at runtime to make appropriate behavioral decisions. In this paper, we present a framework that enables the implementation of an online capability monitor. We derive a graphical system model that captures the relationships between the quality of system elements across different architectural views. In an expert-driven approach, we parameterize Bayesian Networks based on this structure using Fuzzy Logic. Using the online monitor, we infer the quality of the system's capabilities based on technical measurements acquired at runtime.

==> code/define_listings.tex <==
%
\definecolor{delim}{RGB}{20, 105, 176}
\definecolor{numb}{RGB}{20, 105, 176}
\definecolor{punct}{RGB}{20, 105, 176}

\lstdefinelanguage{json}{
    %
    %
    %
    %
    %
    %
    %
    %
    %
    literate={
        {begin}{{{\color{accessblue}{begin\;\,}}}}{1}
        {if}{{{\color{accessblue}{if\;\,}}}}{1}
        {&}{{{\color{accessblue}{\&\;\,}}}}{1}
        {==}{{{\color{accessblue}{==\;\,}}}}{1}
        {then}{{{\color{accessblue}{then\;\,}}}}{1}
    }
}

\lstset{frame=single,
    language=json,
    aboveskip=1mm,
    belowskip=1mm,
    showstringspaces=false,
    columns=flexible,
    basicstyle={\footnotesize\ttfamily},
    numbers=none,
    numberstyle=\tiny\color{gray},
    keywordstyle=\color{accessblue},
    commentstyle=\color{gray},
    stringstyle=\color{mauve},
    breaklines=true,
    breakatwhitespace=true,
    tabsize=4
}

==> code/rule_file.tex <==
\begin{figure*}[!t]
    %
        \begin{lstlisting}[language=json, firstnumber=1]
        longitudinal_control begin
            if estimate_motion == good  & decelerate == pgood & accelerate == bad then bad
            if estimate_motion == pgood & decelerate == good  & accelerate == good then pgood
            if estimate_motion == pbad  & decelerate == good  & accelerate == good then pbad
            ...
        end
        accelerate begin
            if powertrain_actuation == good  then good
            ...
        end
        powertrain_actuation begin
            if power_1 == bad & power_2 == good & power_3 == good & power_4 == good then pgood
            if power_1 == bad & power_2 == good & power_3 == bad  & power_4 == good then pbad
            ...
        end
        \end{lstlisting}
    %
    \caption{Extract of the rule file ``\emph{scenario\_followspeed.rules}''
        defined by experts for the \emph{follow speed} maneuver
        in the example scenario in \autoref{sec:eval}.
        The values \emph{pgood} and \emph{pbad} refer to the states $\pgood$ and $\pbad$.
        \emph{power\_*} denotes the four powertrain units.
    }
    \label{fig:rule_file}
\end{figure*}

==> content/00_keywords.tex <==
\begin{keywords}
    Automated driving, capabilities, monitoring
\end{keywords}

==> content/05_quality.tex <==
%
%
\begin{figure}[H]
    \vspace{-0.55em}
    \centering
    \includegraphics[page=7, width=1.0\columnwidth, height=4.35cm]{figures/unicaragil.pdf}
    \vspace{-1.15em}
    \caption{%
        A graph displaying the interdependencies between the quality of elements
        across different architectural views for the longitudinal \qemph{stop} and \qemph{follow speed} maneuver.
        The latter requires additional capabilities, i.e., nodes and edges indicated by dashed lines.%
    }
    \label{fig:capcomp}
\end{figure}
%
\subsection{Deriving the Graph Representation} \label{sec:quality}
%
Although the elements of different architectural views have a different semantic,
we claim that they are comparable in terms of their quality.
I.e., we suggest that the abstract quality of a capability can be mapped
to the quality of elements in the functional and logical view.
Accordingly, we define a system model that incorporates the qualities
across different architectural views as well as the relations between them.
We define it as a DAG where the nodes represent the \emph{quality states} $Q_i$
of the system elements and the edges represent the correspondences between them.
In general, $Q_i$ can be time-variant and vector valued.
In this work, we focus on the scalar case.

Here, the derivation of the DAG is a hand-tuned expert-based procedure.
The resulting model is shown in \autoref{fig:capcomp}. %
We continue our previous example: %
As mentioned before, in order to control its motion,
the automated vehicle must also have the capabilities ``accelerate'', ``decelerate'' and ``estimate motion''
for which we introduce the quality states
$Q_{\mathrm{Control}}$, $Q_{\mathrm{Accelerate}}$, $Q_{\mathrm{Decelerate}}$ and $Q_{\mathrm{Estimate}}$.
Since several functions are contributing to the realization of these capabilities
(motion controller, powertrain and brake actuation and VDSE functions),
we further introduce $Q_{\mathrm{TrajControl}}$, $Q_{\mathrm{Powertrain}}$, $Q_{\mathrm{Brake}}$ and $Q_{\mathrm{VDSE}}$.
The controller is implemented on the ``StemBrain'' ECU with $Q_{\mathrm{StemBrain}}$.
Furthermore, the four wheel-individual electric motors and corresponding power electronics
making up the powertrain yield the quality states $Q_{\mathrm{PowerUnit},k}$.
Their performance is directly influencing the performance of the powertrain.
In terms of the braking functionality,
we further denote the performance of each brake unit as $Q_{\mathrm{HyBrake},k}$
and the state of the hydraulic power unit as $Q_{\mathrm{HyPower}}$.
Both are directly linked to the quality state $Q_{\mathrm{Brake}}$ in the DAG.
The powertrain and brake components rely on the communication that is
provided on the so-called ``SpinalCord'' ECU with state $Q_{\mathrm{SpinalCord}}$.
Finally, we consider the VDSE functionality and
capture the state of the implemented localization filter as $Q_{\mathrm{Filter}}$.

==> tables/tab_cbelief.tex <==
\begin{table}
    \centering
    \caption{$\cbeh$ for specific distributions of beliefs in $\vpi$, $w = 0.33$}
    \begin{tabular}{p{0.5\columnwidth} | p{0.4\columnwidth}} %
        \toprule        
            $\vpi = (1, 0, 0, 0)^T$ & $\cbeh = 100\perc$ \Bstrut \\
            \hline
            $\vpi = (0.5, 0.5, 0, 0)^T$ & $\cbeh = 83\perc$  \Tstrut\Bstrut \\
            \hline
            $\vpi = (0, 1, 0, 0)^T$ & $\cbeh = 67\perc$  \Tstrut\Bstrut \\
            \hline
            $\vpi = (0.25, 0.25, 0.25, 0.25)^T$ & $\cbeh = 50\perc$  \Tstrut\Bstrut \\
            \hline
            $\vpi = (0, 0, 1, 0)^T$ & $\cbeh = 33\perc$  \Tstrut\Bstrut \\
            \hline
            $\vpi = (0, 0, 0.5, 0.5)^T$ & $\cbeh = 17\perc$  \Tstrut\Bstrut \\
            \hline
            $\vpi = (0, 0, 0, 1)^T$ & $\cbeh = 0\perc$   \Tstrut\Bstrut \\
            %
        \bottomrule
    \end{tabular}
    \label{tab:cbelief}
\end{table}

==> tables/tab_measures.tex <==
\begin{table*}[t]
    \centering
    \caption{Selected technical quality measures and determinants for the components of the ADS-equipped \unicar\ vehicle}
    \begin{tabular}{p{0.25\textwidth} p{0.3\textwidth} p{0.35\textwidth}}
        \toprule        
            Technical Component & Associated Function & Technical Quality Measures \\ \midrule
            Power Electronics & & Maximum power, current and/or voltage, temperature \\
            Wheel-individual electric motors &  & Maximum torque and/or power, positioning accuracy, actuation delay, temperature \Bstrut \\
            \hline
            Hydraulic brake unit 1 & Brake actuation & Maximum brake pressure, actuation latency, temperature \Tstrut\Bstrut \\
            Hydraulic brake unit 2 & Brake actuation & Maximum brake pressure, actuation latency, temperature \Tstrut\Bstrut \\
            Hydraulic power unit & Brake actuation & Available hydraulic pressure, temperature \Tstrut\Bstrut \\
            \hline
            GNSS sensor system & \multirow{2}{10em}{Global localization and state estimation} & Standard deviation of position, latency \Tstrut \\
            IMU-based localization data fusion & & Standard devi ation of position, acceleration, velocity \\
            %
            Electronic control units (ECUs) & -- & Availability, latency, temperature \\
        \bottomrule
    \end{tabular}
    \label{tab:measures}
\end{table*}
